A GP-based Robust Motion Planning Framework for Agile Autonomous Robot Navigation and Recovery in Unknown Environments

For autonomous mobile robots, uncertainties in the environment and system model can lead to failure in the motion planning pipeline, resulting in potential collisions. In order to achieve a high level of robust autonomy, these robots should be able to proactively predict and recover from such failures. To this end, we propose a Gaussian Process (GP) based model for proactively detecting the risk of future motion planning failure. When this risk exceeds a certain threshold, a recovery behavior is triggered that leverages the same GP model to find a safe state from which the robot may continue towards the goal. The proposed approach is trained in simulation only and can generalize to real world environments on different robotic platforms. Simulations and physical experiments demonstrate that our framework is capable of both predicting planner failures and recovering the robot to states where planner success is likely, all while producing agile motion.

==> approach_old.tex <==
\section{Approach}\label{sec:approach}

We propose a GP regression-based scheme to asses the risk of future path planning failure while tracking a trajectory $\bm{\tau}$. Data are collected from simulations that record path planning successes and failures in various states that the robot may encounter during typical operation. This data are used to train a GP regression model to predict the probability of path planning failure for individual states over a future horizon while tracking a trajectory $\bm{\tau}$. The risk of path planning failure over a predicted future horizon of states $\left\{\hat{\bm{x}_i}\right\}$ can then be inferred from these individual future state statistics. Finally, if this risk of future path planning failure exceeds a user-defined threshold, the robot stops tracking $\bm{\tau}$ and a recovery behavior is triggered that finds a state from which the risk of path planning failure is low. We leverage the same GP regression model to ensure a high probability of path planner success from this recovery state.
% This data includes success or failure from a particular state, $Z_{\bm{x}}\in\{0,1\}$, as well as a feature vector $\eta$ that only contains information available to the robot at time $t_0$, specifically the robot state $\bm{x}$ and map $\bm{m}$. This data is used to infer the probability on path planner failure dependent on value of the feature vector, $P(Z_{\bm{x}}|\eta)$
% This data is used to train a model to infer the probability of path planning failure While the low-level is tracking a trajectory $\bm{\tau}(t)$ from the motion planner, model to monitor the probability of failure for individual future states $Z_{\bm{x}_i}$ over a horizon. Statistics from these individual future states are used to infer statistics on the total number of collisions over the future horizon, $Z_{\bm{x}_i}$.
% , and trigger a transition into the recovery mode. During recovery, the robot stops executing $\bm{\tau}(t)$, and leverages the same GP model to find a recovery state $\bm{x}_r$ to navigate towards to continue with nominal operation.

Fig.~\ref{fig:approach_diagram} shows the outline of our approach. The path planner policy $\Pi$ creates a trajectory $\bm{\tau}$ for the low-level controller to track. 
\begin{figure*}[ht!]
    \centering
    \includegraphics[width=.98\textwidth]{main/figs/block_diagram_horiz.png}
    \caption{Block diagram for the proposed approach. }
    \label{fig:approach_diagram}
\end{figure*}
\NB{right side of the diagram inside the green block is not clear HOW the Y and N work}
In our approach, a Model Predictive Controller (MPC) is used to generate the control signal $\bm{u}$ to track $\bm{\tau}$. In doing so, the MPC additionally generates a predicted horizon of future robot states $\left\{\hat{\bm{x}_i}\right\}$ over a prediction horizon $T_F$. These states are used to predict the risk of path planning failure $\rho_{\bm{\tau}}$. If this risk exceeds a user-defined threshold $\psi_\rho$, then the recovery behavior is triggered.
% In this section we will first go over the underlying motion planner used in this work. We will then discuss the novel framework we have developed to both predict and recover from planner failures autonomously.
% In this section we will first go over the underlying motion planner used in this work. We will then discuss the novel framework we have developed to both predict and recover from planner failures autonomously.
To provide a complete description of the approach, Sec.~\ref{subsec:preliminaries} describes the path planning paradigm used in this work, followed by Sec.~\ref{subsec:failure_modes} that explores different modes of path planning failure. Sec.~\ref{subsec:gp_backend} describes how our approach addresses the more challenging task of back-end failure prediction using a GP-based regression model to infer risk of failure $\rho_{\bm{\tau}}$ along the prediction horizon provided by the MPC. Finally, Sec.~\ref{subsec:recovery} describes the recovery behavior that is triggered if this risk exceeds some threshold value, avoiding potential unsafe path planning failures.

\subsection{Path Planner Preliminaries} \label{subsec:preliminaries}
\NM{Collect everyone's thoughts about reducing this section to the bare minimum, discussion of front-end vs back-end.} The planner used in our approach follows the common design paradigm in motion planning of a front-end search followed by back-end optimization for the final trajectory. The front-end search, shown in Fig.~\ref{fig:front_end}, finds a shortest path through free space from the vehicle state $\bm{x}(t_0)$ to the goal $\bm{x}_g$, then expands the path into an intersecting corridor of polytopes $\mathcal{C}$ in free space. The back-end, shown in Fig.~\ref{fig:back_end}, then handles the generation of the final trajectory $\bm{\tau}$.
\begin{figure*}[ht!]
    \centering
    \subfigure[front-end]{\includegraphics[width=0.23\textwidth]{main/figs/dead_end_front_end.png}\label{fig:front_end}} 
	\subfigure[back-end]{\includegraphics[width=0.232\textwidth]{main/figs/dead_end_back_end.png}\label{fig:back_end}}
	\subfigure[failure detection]{\includegraphics[width=0.237\textwidth]{main/figs/dead_end_detection.png}\label{fig:fail_detect}}
	\subfigure[recovery]{\includegraphics[width=0.234\textwidth]{main/figs/dead_end_recovery.png}\label{fig:recovery_execute}}
    \caption{A demonstration of the receding horizon motion planner and recovery pipeline used in this paper. For $\bm{\tau}(t)$, brighter colors denote higher speeds.}
	\label{fig:planner_demonstration}
\end{figure*}

\subsubsection{Planner Front-End}
The front-end starts with the global occupancy map $\mathcal{M}$, which is generated by fusing data from an onboard depth sensor, along with the current state of the vehicle, $\bm{x}(t_0)$, and the goal state $\bm{x}_g$. As shown in Fig.~\ref{fig:front_end}, an initial 0-order path within the free and unknown space of $\mathcal{M}$ is generated by using a graph-based, global planner. In this work, we use the Jump Point Search (JPS) algorithm, as it is a common choice among safe corridor planners due to the reduced computational complexity when compared to other common algorithms like A$^*$ \cite{liu2017sfc}. 
% Note that the global path does not necessarily reach $\bm{x}_g$, and instead plans up to $\bm{x}^*_g$, which is a  distance $\Delta_p$ along the JPS path from $\bm{x}(t_0)$. This is done to prevent the planner from trying to generate infeasibly long trajectories to $\bm{x}_g$ when it is far away.
% More details about $\Delta_p$ and how it is computed are discussed in \ref{subsec:frontend_failure}.

After generating the initial path, a corridor $\mathcal{C}$ of intersecting convex polytopes are established along it in order to connect $\bm{x}(t_0)$ to $\bm{x}_g$. Each polytope $C_i \in \mathcal{C}$ is represented as an H-polytope defined by a matrix $\bm{A}_i$ and vector $\bm{b}_i$ that define a convex set of points $\bm{p}\in\mathbb{R}^2$ in the $xy$ plane
\begin{equation}
    C_i = \{\bm{p} \in \mathbb{R}^2 \, | \, \bm{A_i}\bm{p} \leq \bm{b_i} \}. \label{eq:h_poly}
\end{equation} 

In order to generate each $C_i$ of the corridor $\mathcal{C}$, we rely on the gradient-based optimization approach in \cite{wang2022minco}. We opted for this method as it was empirically seen to produce high coverage corridors using fewer polytopes than other common methods like \cite{tordesillas2021faster}. With $\mathcal{C}$ constructed, the corridor is sent in conjunction with the initial and goal states $\bm{x}(t_0)$ and $\bm{x}_g$ to the back-end optimization in order to find the final trajectory $\bm{\tau}(t)$.

\subsubsection{Planner Back-End}
We represent the trajectory $\bm{\tau}(t)$ (shown in Fig.~\ref{fig:back_end}) as a collection of $N$ time-parameterized polynomials. We use B\'ezier curves to represent these polynomials since they are a commonly utilized basis with several salient properties for corridor-based motion planners.
% which will be discussed in detail after defining the curves formally.
For a background on B\'ezier curves for motion planning, we refer the reader to \cite{gao2018marching}.

% The total trajectory $\bm{\tau}(t)$ is defined by a collection of $N$ B\'ezier curves, $\bm{\tau}_j(t), \, j \in [1,N]$, each defined on the time interval $t \in [0,\Delta t]$ and expressed as: 
% \begin{equation}
%     \bm{\tau}_j(t) = \sum_{i=0}^n \bm{q}^i_j B_n^i(t),
% \end{equation}
% where $n$ is the degree of the curve, $\bm{q}^i_j$ is the $i$th control point, and $B_n^i(t)$ represents the Bernstein polynomial basis \NM{May end up citing \cite{gao2018marching} for the reader to refer to for the theory behind this type of planning scheme instead of discussing it here. }:
% \begin{equation}
%     B_n^i(t) = \binom{n}{i}t^i (1-t)^{n-i}
% \end{equation}

In this paper, we use the cubic ($n=3$) B\'ezier curve for each segment $\bm{\tau}_j(t)$, as it is capable of generating smooth, trackable trajectories for autonomous vehicles. One useful property of the B\'ezier curve $\bm{\tau}_j(t)$ is that it is fully contained within the simplex formed by the control points $\bm{q}^i_j, \, i \in [0,n]$. Thus, for $\bm{\tau}_j(t)$ to be contained within a convex polytope $C$, it is sufficient to ensure that $\bm{q}_j^i \in C, \, \forall i \in [0,n]$. More formally, let $\bm{Q}^B_j = [\bm{q}_0 \, ... \, \bm{q}_n]$ denote the matrix of B\'ezier control points for segment $j$, and $\bm{A_i}$, $\bm{b_i}$ define the $i$th H-polytope in $\mathcal{C}$ as in \eqref{eq:h_poly}. Then, to ensure the segment $\bm{\tau}_j(t)$ is obstacle free, the control points $\bm{Q}^B_j$ of the segment $\bm{\tau}_j(t)$ must be contained within the hyperplanes of the H-Polytope:
\begin{equation}
    \bm{A}_i\bm{Q}_j \leq \bm{b}_i.
\end{equation}

However, the simplex formed from the points in $\bm{Q}^B_j$ often do not tightly bound the curve, and as a result can lead to conservative trajectories or result in the solver failing to find a solution. To resolve this, our approach leverages the minimum volume (MINVO) basis from \cite{tordesillas2022minvo} to convert the B\`ezier curve control points $\bm{Q}^B_j$ into the more tightly bounding MINVO control points $\bm{Q}^{M}_j$. The relationship between the two sets of control points is as follows:
\begin{equation}
    \bm{Q}^{M}_j = \bm{Q}^B_j \bm{K}_B(\Delta t) \left[\bm{K}_M(\Delta t)\right]^{-1},
\end{equation}
where $\bm{K}_B(\Delta t)$ and $\bm{K}_M(\Delta t)$ are conversion matrices for the B\'ezier and MINVO bases respectively, and can be found at \cite{tordesillas2022minvo}. Note that the matrices $\bm{K}$ depend on the current time allocation to the trajectory segments $\Delta t$, thus they must be recomputed when the time allocation is updated in the solver. 

To generate the final trajectory over the horizon, we leverage the FASTER solver  \cite{tordesillas2021faster}, modified to include the MINVO basis to generate a concatenated trajectory $\bm{\tau}(t)$ of $N$ segments in a receding horizon fashion to a specified goal. Once $\bm{\tau}(t)$ has been found, it is sent to the tracking MPC to be executed on the robot.

% \subsection{Receding Horizon Planning}
% \NM{These are implementation details, can be removed if desired.}\NB{yes} We run the control loop at a frequency of $f_c$, which is responsible for running both the front and back-ends of our planner to generate a new trajectory $\bm{\tau}(t)$. The first time the loop is run, the vehicle's current state $\bm{x}(0)$ is used as the initial state. On subsequent loops, a future point $\delta t$ seconds ahead, $\bm{\tau}(t+\delta t)$ is used, where $\delta t$ is a user-defined parameter. $\delta t$ shouldn't be too small, as the solver must be able to generate a solution before the vehicle reaches $\bm{\tau}(t+\delta t)$. However, it also shouldn't be too large as it will impact the ability of the planner to modify the trajectory near the vehicle when necessary. $\bm{\tau}(t)$ is then sent to a non-linear MPC for tracking. This process is repeated until the vehicle either reaches its goal state $\bm{x}_g$, or the recovery behavior is triggered.

\subsection{Failure Modes: Front-End vs Back-End} \label{subsec:failure_modes}

There are two distinct failure modes of the path planner described in~Sec.\ref{subsec:preliminaries}, both of which will result in $\Pi=\emptyset$: a front-end failure, in which an intersecting corridor $\mathcal{C}$ between $\bm{x}(t_0)$ and $\bm{x}_g$ cannot be found, or a back-end failure, in which the numerical solver fails to generate a trajectory along the JPS search path. Front-end failures can occur when a feasible search path doesn't exist (e.g., either $\bm{x}(t_0)$ or $\bm{x}_g$ overlap occupied space within $\mathcal{M}$), or when parameters of the JPS are poorly conditioned for generating a corridor $\mathcal{C}$ (e.g., $|\mathcal{C}|$ is high because the planning horizon distance is too large). The front-end of the path planner implemented in Sec.~\ref{subsec:preliminaries} typically runs in $< 1$ms, thus for a given state $\bm{x}$ and map $\mathcal{M}$, front-end failures are easily determined by simply running the JPS and corridor generation at that state. 

Much more difficult to predict, however, are failures at the back-end of the path planner. Since it is based on a nonlinear optimizer, it can be difficult to characterize success or failure prior to actually running the back-end solver. Additionally, the time to run the back-end is typically $>100$ms, which is too large to directly test multiple future points for failure. Fig.~\ref{fig:fail_detect} shows an example back-end failure mode, in which the discovery of a previously unknown wall (shown as undiscovered space in Fig.~\ref{fig:back_end}) drastically changes the feasible corridor $\mathcal{C}$. The front-end JPS is able to find a feasible path (bright green line), but the back-end is unable to use this warm start to find a feasible trajectory. 

To concretely define these ideas, let $Z_{\bm{x},\mathcal{C}}\in\left\{0,1\right\}$ represent a success ($0$) or failure ($1$) of the path planner pipeline, with $Z^f$ representing a front-end failure and $Z^b\in\left\{0,1\right\}$ representing a back-end failure. Success of the back-end is dependent on success at the front end, and failure of the front-end is interpreted as a failure of the back-end as well, so that $P\left(Z^b=1|Z^f=1\right)=1$. The probability of entire pipeline failure can be written as
\begin{equation}\label{eq:prob_total_failure}
    P(Z_{\bm{x},\mathcal{C}}) = P\left(Z^b|Z^f\right)P\left(Z^f\right).
\end{equation}
The probability of front-end failure is easily and rapidly checked by running the JPS for a given $\bm{x}$ and $\mathcal{C}$, so that effectively $P(Z^f)\in\left\{0,1\right\}$. Our contribution is in estimating $P(Z^b|Z^f=0)$, the probability of back-end failure after a front-end success. For simplicity in notation, the rest of the paper we will write this probability as $P(Z^b)$ and drop the dependence on the front-end outcome.

% Up to this point, the vehicle has been tracking the generated trajectory $\bm{\tau}(t)$ received from the motion planner in order to navigate towards $\bm{x}_g$. However, due to random disturbances and occluded obstacles, $\bm{\tau}(t)$ may intersect with the obstacle space $\mathcal{X}_O$, as in Fig.~\ref{fig:recovery_detection}. Because of this, it is necessary for the vehicle to reason about the environment and current path to predict these planning failures and switch into a recovery mode in order to avoid collisions, as shown in Fig.~\ref{fig:recovery_navigation}. To perform such predictions, the vehicle must be able to assess the likelihood of both front and back-end failures. In this section we will discuss front-end failure detection, and then move on to back-end failures in the following section.

% The process of predicting front-end failure is straightforward, since the runtime is low enough to be executed at several candidate states at runtime \NM{perhaps add some numbers or figure showing the low runtime of front-end vs long runtime of back-end?}. For each state of the tracking MPC horizon $\hat{\bm{x}}(t:t+T) = \left[\hat{\bm{x}}(t), \dots, \hat{\bm{x}}(t+T)\right]$, we run the front-end corridor generation process. If the front-end fails to generate a corridor for a given state $\hat{\bm{x}}(i) \in \hat{\bm{x}}(t:t+T)$, then it is considered to be a failure. This often happens when the state overlaps occupied space in $\mathcal{M}$, since the JPS cannot run if either the start or goal state are occupied. Another common failure mode is that the corridor generation algorithm in \cite{wang2022minco} fails to generate intersecting polytopes. 

% Another common failure mode for the front-end is that the planning horizon distance $\Delta_p$, is too large. This often happens when the generated JPS path to $\bm{x}^*_g$ requires $|\mathcal{P}|$ to be larger than the number of trajectory segments $N$. To prevent this from happening often during nominal planning in more cluttered environments, we warm start the initial $\Delta^{(0)}_p$ to be a user-defined constant $\delta_p$, which is the maximum allowable horizon length for the mission. Then, at the $k$th planning iteration, we update $\Delta^{(k)}_p$ depending on the binary variable $b \in \{0,1\}$, which represents whether the previous planning iteration succeeded ($b=0$) or failed ($b=1$):
% \begin{equation}
% \Delta^{(k)}_p =
%     \begin{cases}
%         \gamma\Delta^{(k-1)}, & \text{if } b = 1\\
%         \max\left[\delta_p, \gamma^{-1}\Delta^{(k-1)}\right] & \text{otherwise } 
%     \end{cases}
% \end{equation}

% Where $\gamma$ is a user-defined constant which controls the aggressiveness at which $\Delta^{(k)}_p$ changes per planning iteration. After running the front-end on each MPC horizon state $\hat{\bm{x}}(i)$, we get success/failure ($b$) for each and collect them into set $\mathcal{B}_f=\{b_t, \dots, b_{t+T}\}$. Once front-end failures are detected, the next step is to detect back-end failure at each state $\hat{\bm{x}}(i)$.
% That is, of the states. where the planner front-end succeeded, predict if the back-end will also succeed at $\hat{\bm{x}}(i)$.

% \begin{figure}[ht!]
%     \centering
%     \subfigure[]{\includegraphics[width=0.23\textwidth]{main/figs/failure_detection.png}\label{fig:recovery_detection}} 
% 	\subfigure[]{\includegraphics[width=0.23\textwidth]{main/figs/recovery_behavior.png}\label{fig:recovery_navigation}}
%     \caption{A demonstration of the failure detection (a) and recovery behaviors (b) using our framework.}
% 	\label{fig:recovery_demonstration}
% \end{figure}

\subsection{Gaussian Process for Predicting Back-End Failure} \label{subsec:gp_backend}

In order to accurately predict back-end failures of the path planning server, we propose a GP-based regression model trained on statistics inferred from simulated data. This data relates the robot and map state to the probability of back-end failure $P(Z^b_{\bm{x},\mathcal{C}})$. A GP model $\hat{P}(Z^b_{\bm{x},\mathcal{C}}|\cdot)$ can be trained to predict probabilities of back-end failure at run time over future states $\{\hat{\bm{x}}_i\}$ provided by the MPC.
% based on a feature vector $\bm{d}(\bm{x},\mathcal{P})$. At run-time, the GP model can be used to quickly predict the probability of a back-end failure ,
These probabilities can then be used to assess the risk of future path planning failure $\rho_{\bm{\tau}}$ over the entire prediction horizon.

A navigation stack comprising of both the path planning policy $\Pi$ and the MPC can be deployed in simulation to gather training examples for the GP model. Each training tuple contains three pieces of information: (i) the state of the robot $\bm{x}$, (ii) the corridor $\mathcal{C}$, and (iii) a binary variable $Z^b_{\bm{x},\mathcal{C}}$ that encodes a success or failure of the path planning back-end. With this data, statistical inferences can be made that relate the robot state and corridor to the probability of back-end failure $P(Z^b_{\bm{x},\mathcal{C}})$. In order to keep inference times low, both robot and map information were distilled into a vector $\bm{d}$ that encoded the salient features needed to accurately predict $P(Z^b_{\bm{x},\mathcal{C}})$. Through study of various possible features that could be used, we found two which were particularly well-suited to predicting the probability of back-end failure: $t_C$, the minimum time-to-intersect (TTI) from robot state $\bm{x}$ to corridor $\mathcal{C}$, and $|\mathcal{C}|$, the number of polygons that defined the corridor. For more details about feature selection and data collection, refer to Sec.~\ref{sec:simulation}.

% The goal of our approach is to construct a model which can enable the motion planner to detect failures in both the front-end corridor construction and back-end optimization proactively and, if necessary, execute recovery behaviors to avoid potential collisions caused by such failures. This problem of anticipating and detecting failures proactively is challenging, as planner failure depends on the characteristics of the environment, the latter of which is unknown a-priori. With this in mind, our approach utilizes a GP classification model which has learned from user-selected characteristics to proactively detect back-end failures.

% Predicting failures in the back-end optimization from a given initial state $\bm{x}_0$, goal state $\bm{x}_g$, and corridor $\mathcal{P}$, can be formulated as a binary classification problem on $b$. Exactly predicting back-end failures can be expensive, especially when considering a set of states within a horizon $T$. This is because the back-end would need to be run at each point separately, which becomes untenable at runtime as the back-end execution time is on the order of $100$ms. For this reason, we use a GP to find an estimate of $b$, denoted as $\hat b = GP(\bm{d})$, which represents the probability of back-end failure $P(b)$ given an input feature vector $\bm{d}$.

% In order to get the GP to predict $\hat{b}$ accurately given $\mathcal{P}$, along with initial and goal states $\bm{x}_0$ and $\bm{x}_g$, the feature vector $\bm{d} \in \bm{D}$ must be a carefully selected set of representative input parameters. 
% We cannot use the corridor and state inputs directly, as their dimensionality would make the problem intractable at runtime for the GP, and would require an abundant amount of training data and a more complex model. \NM{This paragraph needs work...}
% To find such a feature vector $\bm{d}$, we pick out two parameters which were found empirically through collected simulation data and correlate well with failure. The first is $t_P$, the time to intersect (TTI) the boundary of $P_0 \in \mathcal{P}$, the H-polytope enclosing the initial state $\bm{x}_0$.

The minimum TTI can be found by using $\bm{x}$ to calculate the $xy$ position $\bm{p}\in\mathbb{R}^2$ an velocity $\bm{v}\in\mathbb{R}^2$  of the robot, then using kinematic equations to find the minimum TTI of the hyperplanes that define the polytope~$C$ containing $\bm{x}(t_0)$. Formally, if row $\bm{r}_i \in \bm{A}$ and $b_i \in \bm{b}$ form a hyperplane $\bm{r}_i\cdot \langle x,y \rangle -b_i =0$ of polytope $C$,
% along with state $\bm{x}^T=[\bm{p}^T \bm{v}^T \bm{a}^T \bm{j}^T]$, $t_P$ can be calculated via the following function:
then the time to intersect the hyperplane $t_H$ can be calculated as:
% \begin{equation}
%     t_H(\bm{r}_i, b_i, \bm{x}) = \frac{-\bm{r}_i\cdot\bm{p}-b_i}{\bm{r}_i\cdot\bm{v} + \epsilon}, \label{eq:tti}
% \end{equation}
\begin{equation}
t_H\left(\bm{r}_i, b_i, \bm{x}\right) =
    \begin{cases}
        \frac{-\bm{r}_i\cdot\bm{p}-b_i}{\bm{r}_i\cdot\bm{v}} & \text{if } \bm{r}_i \cdot \bm{v} > 0\\
        \gamma_t & \text{otherwise}
    \end{cases}
\end{equation}
where $\gamma_t$ is a user-defined maximum value for $t_H$ when the vehicle is stationary or moving away from the hyperplane. 
% A small $\epsilon$ term is added in the denominator to limit $t_H$ when $\|\bm{v}\|_2 \approx 0$. Since $t_H < 0$ when the vehicle is moving away from the hyperplane, all $t_H \geq 0$ are added to $\mathcal{T}_C=\left\{t_H \, | \, t_H \geq 0\right\}$, the set of all non-negative TTI for polytope $C$. From $\mathcal{T}_C$, the minimum TTI is found by finding the smallest TTI in the set: $t_C=\min\left(\mathcal{T}_C\right)$. \NM{come back and explain this better.} 
From $t_H$, the time to intersect polytope $C$, $t_C$, is defined as the minimum TTI to one of its hyperplanes:
\begin{equation}
    t_C = \argmin_i \{t_H\left(\bm{r}_i, b_i, \bm{x}\right)\}.
\end{equation}

One of the biggest factors that affect the ability of the back-end solver to find a feasible solution is how close the current robot state $\bm{x}$ is located to the boundary of the feasible set $\mathcal{C}$. Intuitively, TTI is an effective predictor of back-end failure because it captures several factors determining success: 1) The physical distance between the state $\bm{x}$ and the boundary of the solver, 2) the speed of the robot, 3) the heading of the robot.

In addition to TTI, the cardinality $|\mathcal{C}|$ of the corridor also plays a role in failure of the back-end solver: if $\mathcal{C}$ is defined by many polytopes, then obstacles in the environment necessitate a very non-direct path to be planned for the robot, further complicating the search for a feasible path.
% Through data collection, it was found that the ratio of failures increased as $t_P \rightarrow 0$, shown in Fig.~\ref{fig:tti_data}(a), thus indicating that it is a reasonable parameter to include in the model input.
Together, these two features were used inside a feature vector $\bm{d}(\mathcal{C},\bm{x})=\left[t_C,|\mathcal{C}|\right]$ to infer the probability of back-end failure. To find this probability, the back-end failure training data $\left\{Z^b_{\bm{x},\mathcal{C}}\right\}$ were binned based on feature vector value $\bm{d}$, and ground-truth probability of failure $P(Z^b_{\bm{x},\mathcal{C}})$ was found within each bin.
In general, both a smaller TTI and a larger corridor set length leads to a higher probability of back-end failure.
% For more discussion about feature extraction and correlation, refer to Sec.~\ref{sec:simulation}

% The second parameter used is $|\mathcal{P}|$, the size of the generated corridor. This parameter is added to the feature vector as it also shows a trend with solver failure: the more polytopes in the corridor, the higher the ratio of failures (see Fig.~\ref{fig:tti_data}(b)). Thus, the final input feature vector used in our approach is $\bm{d}(\mathcal{P}, \bm{x})=\left[t_P(\bm{A}_0, \bm{b}_0, \bm{x}), \left|\mathcal{P}\right|\right]$. For more information about training the model and data collection, refer to the simulation discussion in section \ref{sec:simulation}. 

The underlying GP model input is defined by a collection of $M$ input training features, $\bm{D}=\left[\bm{d}_0, \dots, \bm{d}_M\right]$, and values $\bm{P}=\left[P_0, \dots, P_M\right]$, with an output defined by a joint Gaussian distribution  \cite{rasmussen2005gaussian}:
\begin{equation}
    \begin{bmatrix} P \\ \hat{P} \end{bmatrix} \sim \mathcal{N}\left( \begin{bmatrix} \mu(\bm{d}) \\ \mu(\bm{d}_*) \end{bmatrix}, \begin{bmatrix} \bm{K} & \bm{K_*} \\ \bm{K}_*^T & \bm{K_{**}} \end{bmatrix} \right), \label{eq:gp}
\end{equation}
where $\bm{K}=\kappa(\bm{D}, \bm{D})$, $\bm{K_*}=\kappa(\bm{D},\bm{D}_*)$ and $\bm{K_{**}}=\kappa(\bm{D}_*, \bm{D}_*)$, $\mu$ is the mean function, $\bm{D}_*$ is the test input, and $\kappa$ is a positive definite kernel function, which is the commonly used Matern covariance function in this work. From this, the predictive posterior distribution of $\hat{P}$ given the training data $\bm{D}$ can be expressed as another Gaussian distribution:
\begin{equation}
    \hat{P} \sim \mathcal{N}(\mu_*, \sigma_*^2),
\end{equation}
with $\mu_*$ and $\sigma_*^2$ defined as:
\begin{equation}
    \mu_* = \mu(\bm{D_*}) + \bm{K}_*^T\bm{K}(P-\mu(\bm{D}))
\end{equation}
\begin{equation}
    \sigma_*^2 = \bm{K}_{**}-\bm{K}_*^T\bm{K}^{-1}\bm{K}_*.
\end{equation}
Finally, the estimated probability of back-end failure is taken as the mean values of this posterior:
\begin{equation}
    \hat{P}(Z^b_{\bm{x},\mathcal{C}}|\bm{d}) = \mu_*.
\end{equation}

% Since front-end planner failures were already tested prior, the back-end GP prediction only needs to be run on those MPC states $\hat{\bm{x}}(i)$ where the front-end succeeded: $\hat{b}_i = 0, \, \hat{b}_i \in \mathcal{B}_f$. Note that in the case of front-end success and failure, $\hat{b}_i$ can be known with certainty to be either $0$ or $1$. \NM{Re-assess the formulation of this part} Running the GP on those states and combining with $\mathcal{B}_f$ will yield a final set $\mathcal{B} = \{\hat{b}_t, \dots, \hat{b}_{t+T}\}$ which denotes the predictions of planner failure (either front or back-end) over the MPC horizon $\hat{\bm{x}}(t:t+T)$.
% After running the MPC horizon states $\hat{\bm{x}}(i)$ which succeeded in front-end planning through the GP, we get the back-end failure predictions at each state $\hat{\bm{b}}$. Finally, we construct 

With $\hat{P}(Z^b_{\bm{x},\mathcal{C}}|\bm{d})$ estimating back-end failure, the probability of failure for the entire path planning pipeline $P(Z_{\bm{x},\mathcal{C}})$ can be calculated using~\eqref{eq:prob_total_failure}. These probabilities can be used to infer the risk of path planning failure along the future states $\left\{\hat{\bm{x}}_i\right\}$ predicted by the MPC. To formulate this risk, we consider the total number of future path planning failures $Z_{\bm{\tau}}$ as the salient outcome to track, defined as
\begin{equation}
    Z_{\bm{\tau}} = \sum_{\hat{\bm{x}} \in \{\hat{\bm{x}}_i\}}Z_{\hat{\bm{x}},\mathcal{C}}.
\end{equation}
Because each $Z_{\hat{\bm{x}},\mathcal{C}}$ is a stochastic variable, so too is $Z_{\bm{\tau}}$. The risk metric chosen in our approach is the expected number of collisions over the future horizon, $\rho_{\bm{\tau}} = \mathbb{E}(Z_{\bm{\tau}})$. The expected value is chosen here for its simplicity and speed to calculate, although other risk metrics may be used as well. Since each $Z_{\hat{\bm{x}},\mathcal{C}}$ is a Bernoulli random variable with predicted probability $\hat{P}(Z_{\hat{\bm{x}},\mathcal{C}}|\bm{d})$ of failure, the expectation is calculated as \NM{We should consider putting hats over this $P$, given that it is an estimate of the true probability}:
\begin{equation}
    \rho_{\bm{\tau}} = \sum_{\hat{\bm{x}} \in \{\hat{\bm{x}}_i\}} P(Z_{\hat{\bm{x}},\mathcal{C}}).
\end{equation}

A risk threshold $\psi_\rho$ may be set so that anytime the risk of planner failure over future states $\left\{\hat{\bm{x}}_i\right\}$ exceeds this value, a recovery behavior is triggered to prevent this planner failure. 
% \NM{Following formulation definitely needs some work, the b's are getting out of hand}With the GP model trained, the states along the MPC horizon $\hat{\bm{x}}(t:t+T)$ are passed in to the GP. Doing so yields the collection of predictions for back-end failure $\mathcal{B}_b = \{\hat{b}_t, \dots, \hat{b}_{t+T}\}$. Since $\mathcal{B}_f$ and $\mathcal{B}_b$ both contain the probabilities for front and back-end failures, they can be rounded to obtain the predicted failure labels $b\in \{0,1\}$. The two sets can then be concatenated with an element-wise OR operation to produce $\mathcal{B}$, which denotes the prediction of planner failure at each state of the MPC horizon $\hat{\bm{x}}(t:t+T)$. We use the OR operation due to the fact that either front or back-end failure is sufficient for overall planner failure.



% , we run the GP model at each state of the MPC horizon $\bm{x}(t:t+T)=[\bm{x}(t_0), \dots, \bm{x}(t+T)]$ which tracks the current trajectory $\bm{\tau}(t)$.
% From $\mathcal{B}$, we compute the failure score, $\sigma_f$ by checking if $N_f$ failures occur consecutively in the horizon: 
% \begin{equation}
%     \sigma_f = \argmax_{k \in [0,T-N_f]} \prod_{i=k}^{k+N_f} \text{round}(\hat{b}_i)
% \end{equation}
% \begin{equation}
%     \sigma_f = \argmax_{\hat{\bm{b}}_i \in \mathcal{B}} \prod_{i=k}^{k+N_f} \text{round}(\hat{b}_i)
% \end{equation}
% where $N_f$ is a user defined parameter which should be selected based on the vehicle's stopping distance and how conservative the detector should be. In this formulation, $\sigma_f=1$ if the GP predicts $N_f$ consecutive failures along the horizon, which triggers the vehicle to come to a stop in the environment and begin recovery behaviors. 

\subsection{Recovering After Predicted Failures}\label{subsec:recovery}
When $\rho_{\bm{\tau}} > \psi_\rho$ is satisfied, it means that there is a collection of states in the vehicle's future horizon that the planner is likely unable to successfully operate in. As such, the vehicle must stop or perform other recovery maneuvers in order to avoid collisions and navigate successfully through said regions. Unlike prior works where human operators intervene to recover the vehicle once failures are detected \cite{ji2022paad}, \cite{kahn2021land}, our framework also includes a recovery planner $\Pi_r$ which enables the vehicle to find and execute safe recovery maneuvers autonomously, as illustrated in Fig.~\ref{fig:recovery_execute}.

Once the vehicle has stopped after switching to the recovery mode, the objective is to locate a nearby region where the planner will succeed, i.e $Z_{\bm{x},\mathcal{C}}=1$. The first step in this process is to sample points uniformly in free space around the current vehicle position $\bm{p}(t_0)$. In order to do so, we generate an H-polytope $C_{r}$ around $\bm{p}(t_0)$, then use hit-and-run Markov-chain Monte Carlo sampling to find the set of $N_p$ candidate positions $\mathcal{P}_{c} = \{\bm{p}_0, \dots, \bm{p}_{N_p}\}$, where $N_p$ is a user-defined parameter. We then convert $\mathcal{P}_{c}$ to states $\mathcal{X}_{c}$ by assuming the vehicle will start from rest, giving zero vectors for velocity, acceleration, and jerk. We make this choice because it significantly reduces the sample space and sampling only positions was enough to find recovery points in practice. 

With $\mathcal{X}_{c}$, we find the probability of planner failure, $Z_{\bm{x}_i,\mathcal{C}_i}$, at each $\bm{x}_i$. In the event that all predictions have failure probability greater than $\eta$, the samples are thrown away and the sampling process is repeated. Here $\eta$ is a user-defined parameter which controls how risk averse the recovery behavior should be when selecting candidate recovery states. To choose the final recovery point $\bm{x}_r$, the point with lowest expected failure is selected:
\begin{equation}
    \bm{x}_r = \argmin_{\bm{x}_i \in \mathcal{X}_c} \mathbb{E}\left[Z_{\bm{x_i},\mathcal{C}_i}\right]. \label{eq:rec_state}
\end{equation}
% We then add all states $\bm{x}_i$ whose probability of failure were less than a user-defined parameter $\eta$ and add them to the final set of recovery states $\mathcal{x}_r$. In the event where $|\mathcal{x}_r| < N_p$, we continue uniformly sampling in $P_r$ until $N_p$ recovery points are found.
% run each state $\bm{x}_i \in \mathcal{X}_{c}$ through the front-end planner processes with goal $\bm{x}_g$ in order to generate the corresponding corridor $\mathcal{P}_i$. 
% With $\bm{x}_i$ and $\mathcal{P}_i$, the GP input feature $\bm{d}_i$ is constructed and sent through the GP model to obtain and
% Finally, we run each state $\bm{x}_i \in \mathcal{x}_r$ through the following cost-to-go scoring function in order to determine the best recovery point $\bm{x}_r$ to navigate towards:
% In order to determine the final recovery state $\bm{x}_r \in \mathcal{x}_r$ the state $\bm{x}_i \in \mathcal{x}_r$ which maximizes the following scoring function is selected as recovery point $\bm{x}_r$:
% \begin{equation}
%  \Gamma(\hat{b}_i, \bm{x}_i, \bm{x}(t_0)) = \left(1-\hat{b}\right)\left[w_\theta \theta(\bm{x}_i, \bm{x}(t_0)) + \frac{w_d}{d_{max}} d(\bm{x}_i, \bm{x}(t_0))\right],
% \end{equation}
% \begin{equation}
% \Gamma\left(\bm{x}_i, \bm{x}(t_0)\right) = \left[w_\theta \theta(\bm{x}_i, \bm{x}(t_0)) + \frac{w_d}{d_{max}} d(\bm{x}_i, \bm{x}(t_0))\right],
% \end{equation}
% where $\theta(\cdot)$ is a function which computes the normalized heading error between two states, $d(\cdot)$ computes the euclidean distance between two states, and $d_{max}$ is the distance from the current robot state $\bm{x}(t_0)$ to the furthest recovery point in $\mathcal{x}_r$:
% \begin{equation}
%     d_{max} = \argmax_{\bm{x}_i \in \mathcal{x}_r} d(\bm{x}(t_0), \bm{x}_i)
% \end{equation}
%  with highest probability of success is selected as $\bm{x}_r$:
% \begin{equation}
%     \bm{x}_r = \argmax_{\bm{x}_i \in \mathcal{x}_r} GP(\bm{d}_i)
% \end{equation}
% To prevent $\bm{x}_r$ from being set to a state $\bm{x}_i$ with low confidence of success, we set a user defined parameter $\eta$ such that if $\hat{b}_i = GP(\bm{d}_i) < \eta$, the samples are discarded and the process is repeated until a state of high success confidence is found. 
% $\bm{x}_r$ is then selected as the state $\bm{x}_i \in \mathcal{x}_r$ which minimizes $\Gamma(\cdot)$:
% \begin{equation}
%     \bm{x}_r = \argmin_{\bm{x}_i \in \mathcal{x}_r} \Gamma\left(\bm{x}_i, \bm{x}(t_0)\right)
% \end{equation}

After determining $\bm{x}_r$, the vehicle navigates to the recovery point using a go-to-goal MPC with added constraint, formulated as in \eqref{eq:h_poly}, where the vehicle position $\bm{p}(t_0)$ must remain in $C_r$ in order to avoid obstacles.
% The cost function $J(\cdot)$ for this control problem is defined over the horizon $T$ as:
% \begin{equation}
%     J \left(\bm{x}(t_0), \bm{u}(t)\right) = \int_0^T |\bm{x}(t_0)-\bm{x}_g|^2_{\bm{Q}} + |\bm{u}(t)|^2_{\bm{R}} \, dt,
% \end{equation}
% where $\bm{u}(t)$ is the control input and $\bm{Q}$ and $\bm{R}$ are positive definite weight matrices for the state error and control input respectively. In order to ensure the vehicle avoids obstacles in the environment, we add halfplane constraints from $C_{r}$ as defined in \eqref{eq:h_poly} to ensure the vehicle remains inside the polytope while navigating towards $\bm{x}_r$. Thus, the final MPC formulation is as follows:
% \begin{equation}
% \begin{aligned}
%     \min_{u} \quad & J\left(\bm{x}(t_0), \bm{u}(t)\right) \\
%     \textrm{s.t.} \quad & \bm{x}(0) = \bm{x}_0 \\
%     & \dot{\bm{x}} = f(\bm{x}, \bm{u}) \\
%     & \bm{A}_{r}\bm{p} -\bm{b}_{r} \leq \bm{0}
% \end{aligned}
% \end{equation}
Once the vehicle reaches $\bm{x}_r$, the planner switches back to the nominal policy $\Pi$, where the planner runs the front and back-end processes to generate trajectories $\bm{\tau}(t)$ which are then executed by the tracking MPC. 
